Counterspeakers' Perspectives: Unveiling Barriers and AI Needs in the Fight against Online Hate

Counterspeech, i.e., direct responses against hate speech, has become an important tool to address the increasing amount of hate online while avoiding censorship. Although AI has been proposed to help scale up counterspeech efforts, this raises questions of how exactly AI could assist in this process, since counterspeech is a deeply empathetic and agentic process for those involved. In this work, we aim to answer this question, by conducting in-depth interviews with 10 extensively experienced counterspeakers and a large scale public survey with 342 everyday social media users. In participant responses, we identified four main types of barriers and AI needs related to resources, training, impact, and personal harms. However, our results also revealed overarching concerns of authenticity, agency, and functionality in using AI tools for counterspeech. To conclude, we discuss considerations for designing AI assistants that lower counterspeaking barriers without jeopardizing its meaning and purpose.

==> content/backups/03-interview-study.tex <==
\section{Interview Study}
\maarten{Add a sentence or two, to tie this section's purpose to the main RQs of the paper. Maybe give a super high-level overview of what we did /with whom? Also we need to add info on IRB that Cathy got.}
We first conducted semi-structured interviews with experienced counterspeakers to understand counterspeech from participants with diverse experiences countering hate and a more developed identity as counterspeakers. 
We asked questions to understand their counterspeech experiences and thoughts on AI tools, possible benefits and drawbacks, to provide insights into each of our research questions. 

\jenny{Can we turn this into one big section titled "Methodology", with two subsections interview study and survey study? and then turn all the current subsections into subsubsections}
\maarten{That sounds good, but I don't love subsubsections, can we use paragraphs instead?}\jenny{yeah sounds good to me :)}
\maarten{Following up on this: I think we need to make the full methodology section together, and split off into 3.1 Interview study wth and 3.2 Survey study. Then for each study, we should do procedure/questions, and then participants recruitment+demographics, and then analysis methods.}

\jimin{TODO: specify that results are in the findings section}
\subsection{Participants}
% \maarten{This needs to be tidied up and made more research-paper-y. Start with how we got in contact with participants (one of the authors...), then describe their experience with counterspeech?}
Ten participants were purposefully selected based on their long-term experience doing counterspeech online in a systematic way. One of the authors had conducted a previous study with the participants, so recruitment was carried out through direct invitations. The participants come from a variety of backgrounds in different contexts (from Europe, Africa, and North America).  Some counterspeak collectively, while others respond individually. This sampling approach aimed to ensure a diverse range of perspectives and rich data for analysis. All participants provided informed consent prior to their participation and confidentiality and anonymity were maintained throughout the study, with pseudonyms used in reporting findings.

\subsection{Interview Procedure}
\maarten{Need some citations for the methods we used?}
This study employed a qualitative research design, utilizing semi-structured interviews as the primary data collection method. The aim was to gain an in-depth understanding of the challenges counterspeakers face, the strategies they use, and their thoughts about the possibility of using AI to improve their counterspeech. 

To ensure consistency, we developed an interview guide which consisted of open-ended questions designed to explore participants' experiences doing counterspeech and their insights into how AI tools could aid or complicate their work. We chose semi-structured interviews as they allow participants to express their thoughts, experiences, and perspectives, while also providing the flexibility to probe for deeper insights as the conversation unfolds. 

\jenny{Add in some data summarizing relevant features of the population (e.g., gender, years of experience doing counter speech maybe?)}
\subsection{Analysis Method}
Grounded Theory methodology \cite{charmaz2006constructing,glaser1967discovery} was employed to analyze the interview data. This iterative and systematic approach allowed for the discovery and development of theories directly from the data. The analysis process involved three key coding stages: open coding, axial coding, and selective coding. 
\begin{enumerate}
    \item Open Coding: In this initial stage, each interview transcript was thoroughly reviewed, and initial codes were generated by breaking down the data into meaningful units. This process involved line-by-line coding, enabling the emergence of concepts and patterns without preconceived notions.
    \item Axial Coding: Building upon the initial codes, axial coding aimed to establish relationships between codes and identify broader categories and subcategories. This stage helped uncover the connections and interactions within the data.
    \item Selective Coding: The final stage involved refining and integrating categories to develop a coherent theoretical framework. Codes were examined for commonalities and variations, leading to the identification of core concepts and their interrelationships.
\end{enumerate}

Stage one and stage two coding was conducted by the same author who conducted the interviews, as was required by our IRB to protect participant confidentiality. The research team conducted stage three coding together, integrating the findings of both the survey research and the interview study.  
% \subsection{Results}
% hate speech experience
% some themes

==> content/backups/04-survey-study-backup.tex <==
\begin{table}[]
    \centering
    \begin{tabularx}{\textwidth}{llX}
         Question Topic & QId & Question\\
         & &  \\
         & & 
    \end{tabularx}
    \caption{Caption}
    \label{tab:survey-questions}
\end{table}

\section{Survey Study}
To understand a broader user experience with hate speech and counterspeech, we conducted a survey study with participants from Amazon Mechanical Turk (MTurk). 
We recruited participants from a pool of pre-qualified workers using the process detailed in \ref{app:qual}.
We excluded survey results with nonsensical qualitative answers (e.g., repetitive answers, discussing irrelevant technology, or copy and pasted answers from internet sources). 

\jenny{maybe move participants section up to the front to be consistent with the interview section}\maarten{+1}

\subsection{Participant Demographics}
Since we recruited mainly from U.S. and Canada, majority of the participants were from the U.S. (98\%) and many of them identified as white or Caucasian (83\%).
On question about gender identity, 56\% of participants identified as male and 41\% female.
When asked about sexuality, 85\% reported as being straight (heterosexual) followed by bisexual (6\%) and asexual (2\%).
In political spectrum, participants were liberal-leaning with strongly liberal 22\%, liberal 32\%, moderate 18\%, conservative 17\%, and strongly conservative 8\%.
\jimin{todo: correlation / results by demographics? ask in meeting what's important}

\begin{figure*}[htpb]
  \centering
  \subcaptionbox{Hate speech and counterspeech experiences\label{hate-counter-freq}}{%
     \includegraphics[width=0.45\textwidth]{figures/frequency_hate.pdf}%
  }
  \subcaptionbox{Most Commonly Seen Hate Speech Categories\label{subfig:hate-type}}{%
    \includegraphics[width=0.45\textwidth]{figures/hate_type.pdf}
  }
  \caption{Hate Speech and Counterspeech Experience Responses}
  \label{a-two-column-figure}
\end{figure*}

\subsection{Survey Design}
\maarten{this is a little long, can we potentially give high-level picture and list the questions in a table format or enumarated format?}
The survey was designed after initial qualitative interviews reflecting some of the high-level findings such as AI tools discussed by the experienced counterspeakers. 
% We iteratively designed the survey as a research team.
The survey included four main parts: hate speech experience, counterspeech experience, AI tools for counterspeech, and demographics.
In the first part, we asked the participants questions about social media usage and their experiences with hate speech online such as types of hate, platform, and types of online spaces, public or private (5 questions).
The second part of the survey consisted of questions about counterspeech experience. 
More specifically, we asked participants about their responses to hate speech and barriers to responding if they had chosen not to respond (\todo). 
The third part of the survey focused on questions about AI tools. 
To understand how open participants were to AI tools more generally, we asked how likely they would be to use an AI tool that assisted solving the barriers they selected. 
We asked two qualitative questions prior to the quantitative questions about tool preferences to prevent any priming the users with certain types of tools. 
First, we asked participants what the reasons would be to either use or not use an AI tool that addressed their concerns when responding to hate speech. 
Second, we asked participants to envision possible AI tools, if any, that might make them more likely to write a response to hate speech. 
Below is the specific wording for each qualitative question.
\begin{enumerate}
    \item What are the reasons that you are likely or unlikely to use it (an AI tool that addresses the barrier in the previous questions)?
    \item What type of AI assistance do you think would make you more likely to write a reply to hate speech?
\end{enumerate}
In the quantitative portion, we divided tools envisioned by the research team and the experienced counterspeakers into two types: collaborative writing tools for counterspeech and bots, i.e., automated responses. 
\jimin{probably need to remove that some options were from the interview since we don't specify how}
% add something here about the questions that were either choose all that apply or choose three

\subsection{Analysis Method}

\paragraph{Quantitative Responses}
We report the quantitative responses with percentage of participant responses. 
For those questions that asked participants to select all that apply, we counted the number of participants who responded and calculated the percentage.

\jenny{Maybe be more specific about how you calculate the percentage? Are we aggregating similar responses together (e.g., strongly agree, agree)? For each type of Likert response, we could describe which categories we combined together / what we end up reporting in our results in the \%s.}\maarten{+1}

\paragraph{Qualitative Responses}
\maarten{This is quite long, can we break this up into paragraphs, and maybe condense?}
To analyze the qualitative survey responses, we performed open coding on the data. In this analysis, we interpreted generated codes as itemized claims about the data to be investigated in other work and surfaced coding disagreements, following recent best practices in qualitative analysis~\cite{hammer2014confusing}. To open code the data, we first created separate documents containing the survey responses to each question~\cite{saldana2009coding}. Next, two members of the research team first inductively generated codes for 25\% of the data developing individual code books. Each code was given a name along with a short description. Additionally, each instance was labeled with zero or more codes. Next, the authors convened to merge their individual codebooks into a shared codebook. To do so, the authors first identified codes with similar themes and merged these codes into a single code. For the remaining codes, the authors discussed instances of disagreement and unanimously agreed to add, merge, or delete the code. After developing the shared codebook, the authors then performed a second round of coding by deductively applying the codebook to the entire dataset individually. The authors then reconvened to apply the codes. For each instance in the dataset, the authors applied the codes they both agreed upon and discussed the disagreements on others. They added or removed the code from the instance upon unanimous agreement. Disagreements largely occurred due to differing scopes of codes and at times different interpretations of the statements, which were resolved through discussion.

\subsection{Quantitative Results}
\jenny{Can we move this section to findings instead?}

\begin{figure*}[htpb]
  \centering
  \subcaptionbox{Hate speech and counterspeech experiences\label{hate-counter-freq}}{%
     \includegraphics[width=0.45\textwidth]{figures/frequency_hate.pdf}%
  }
  \subcaptionbox{Most Commonly Seen Hate Speech Categories\label{subfig:hate-type}}{%
    \includegraphics[width=0.45\textwidth]{figures/hate_type.pdf}
  }
  \caption{Hate Speech and Counterspeech Experience Responses}
  \label{a-two-column-figure}
\end{figure*}

\paragraph{Online Hate Speech Experiences}
When asked about their online hate speech experiences, overwhelming majority (94\%) of the respondents said they had encountered hate speech online. 
Facebook and Twitter / X were the top two platforms where participants encountered hate speech most frequently although YouTube and Facebook ranked the top weekly used platforms. 
Most participants observed more hate speech in public online spaces (84\%) compared to private.

The types of hate the participants reported seeing most frequently were ``Race-based or Ethnicity-based hate speech'' (56\%) followed by ``Hateful speech against members of a specific political party'' (48\%).
The full rankings of categories of hate are shown in Figure~\ref{subfig:hate-type}. Additional categories of hate encountered and identified by the participants are listed below. Examples of online hate encountered by participants include \jenny{fill this in with participant quotes}
\begin{itemize}
    \item ``against farmers, vegans''
    \item ``Against people with different entertainment preferences''
    \item ``General hatred towards liking certain things, like matters of personal taste''
    \item ``Anti Conservative hate, anti Straight hate, anti male hate''.
\end{itemize}

% \begin{table}[htpb]
%     \centering
%     \small
%     \begin{tabularx}{\textwidth}{Xl}
%         \toprule
%         \textit{Counterspeech Barrier} & \textit{Responses (\%)} \\
%         \hline
%         I did not respond because I didn't think responding would have an impact & 73 \\
%         I did not respond because I didn’t want people to be mad at me or send me hateful or threatening messages & 31 \\
%         I did not write a reply because I did not know what to say & 22 \\
%         I did not write a reply because I didn’t have enough time & 21 \\
%         I did not write a reply because I didn't know how to say what I wanted to say & 17 \\
%         Other & 9 \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Caption}
%     \label{tab:cs-barrier}
% \end{table}

\paragraph{Counterspeech Experiences and Barriers}
As shown in Figure~\ref{hate-counter-freq}, participants responded to hate speech in much lower rate than encountering hate speech.
When participants did respond to hate speech, highest number of participants were primarily responding to ``people that they (I) do not know'' (49\%) and ``equally as an ally and as a member of the targeted group'' (45\%).

% who are they responding to?
The participants responded to hate speech by almost equally commenting or replying directly under the post (72\%) and reacting with downvotes or dislikes (70\%) followed by reporting hateful speech (49\%). 
The participants reported that they have responded by using tactics to ``correct misinformation'' (72\%), ``shame the person who posted hate speech'' (36\%), and ``posted links to trustworthy sources'' (34\%). 
The tactics that participants reported using most often were 
Some other tactics identified by the participants included the following.
\begin{itemize}
    \item ``I think I tend not to post or get involved in a hate speech post.''
    \item ``I like copying their post, but changing the demographic so they can see how bigoted they are.  Such as all the anti-white racism that I see, I will write an exact copy of their post and put "black" where they had the word "white" and suddenly they think it's "racist". It exposes their own biases.''
    \item ``be hateful back''  
\end{itemize}

The most common barrier to responding was ``I did not respond because I didn't think responding would have an impact'' (73\%).
Other barriers (\textit{N=28}) identified by the participants included most notably the following responses. 
\begin{itemize}
    \item \textit{``I would not dignify such vitriol with a response.''} (P54)
    \item \textit{``I did not write a reply because I couldn't be bothered to care about it enough.''} (P98)
    \item \textit{``I did not respond because for the most part people should be able to say what they want. It's up to us whether we choose to be hurt by someone's comments or not.''} (P190)
\end{itemize}

% how are they responding?

% what are the barriers

% \begin{table}[]
%     \centering
%     \small
%     \begin{tabularx}{\textwidth}{Xl}
%         \toprule
%         \textit{Tool Description} & \textit{Preference (\%)} \\
%         \hline
%         An AI tool that suggests facts and quotes to add to your reply & 58 \\
%         An AI tool that suggests fully written countering posts for you to select and post & 44 \\
%         An AI tool that helps you collaboratively write a countering post (e.g. make suggestions, provide grammatical edits) & 39 \\
%         An AI tool that rewrites your response with a different tone and corrections & 32 \\
%         An AI tool you can call to post a response for you (not using your account) & 22 \\
%         Other & 5 \\
%         \bottomrule
%     \end{tabularx}
%     \caption{\maarten{let's make this a barchart too?}}
%     \label{tab:cs-tool}
% \end{table}
\paragraph{AI Tool Preferences}
Openness to AI tool was slightly shifted towards likely (50\%) compared to unlikely (31\%).
More detailed results of AI tool usage preferences are shown in Figure~\ref{subfig:ai-tool}.
When asked about collaborative tools, participants preferred ``An AI tool that suggests facts and quotes to add to your reply'' (58\%) the most and least preferred was ``An AI tool you can call to post a response for you (not using your account)'' (22\%). 
Other tool options and corresponding percentages are shown in Table~\ref{tab:cs-tool}.
Similarly, participants most preferred bots that responded with ``Relevant facts'' (66\%). 
% \subsection{Qualitative Results}

% \paragraph{Benefits of AI Tools}
% likely - similar to the concerns raised about selecting what to respond to, participants were seeking similar hate speech reassessement technology that is unbiased second opinion on whether they are being emotional or not
% - AI have more experience, might be more eloquent than themselves

% maybe rename as reasons against AI tools?
% \paragraph{Concerns about AI Tools}
% inauthentic - not only is it not coming from you, but if you care enough about it, you should write yourself

% \paragraph{Direction of AI Assistance}
% something that can suggest hate speech to respond to in an unbiased way
% in a calm way (help emotionally regulate)
% protects the writer from subsequent engagement and from being the target (anonymous)
% is good at generating factual arguments
% can help understand the impact and understand the hate speaker
% can help figure out if they are actually talking to someone - a real person - vs not 
% ** ignorance as a response **

==> content/backups/04-survey-study.tex <==
\begin{table}[]
    \centering
    \begin{tabularx}{\textwidth}{llX}
         Question Topic & QId & Question\\
         Hate Speech & &  \\
         Counterspeech & & \\
         AI Tools & & \\
    \end{tabularx}
    \caption{Caption}
    \label{tab:survey-questions}
\end{table}

\section{Survey Study}
To understand a broader user experience with hate speech and counterspeech, we conducted a survey study with participants from Amazon Mechanical Turk (MTurk). 
We recruited participants from a pool of pre-qualified workers using the process detailed in \ref{app:qual}.
We excluded survey results with nonsensical qualitative answers (e.g., repetitive answers, discussing irrelevant technology, or copy and pasted answers from internet sources). 

\jenny{maybe move participants section up to the front to be consistent with the interview section}\maarten{+1}

\subsection{Participant Demographics}
Since we recruited mainly from U.S. and Canada, majority of the participants were from the U.S. (98\%) and many of them identified as white or Caucasian (83\%).
On question about gender identity, 56\% of participants identified as male and 41\% female.
When asked about sexuality, 85\% reported as being straight (heterosexual) followed by bisexual (6\%) and asexual (2\%).
In political spectrum, participants were liberal-leaning with strongly liberal 22\%, liberal 32\%, moderate 18\%, conservative 17\%, and strongly conservative 8\%.
94\% of the respondents had experience encountering hate speech online and 70\% had experience responding to hate speech but only 8\% did so frequently or all the time even though 22\% encountered hate speech frequently or all the time. 
The most commonly seen type of hate speech was race-based or ethnicity-based (56\%), and most participants primarily responded either equally as an ally and targeted group (45\%) or as an ally (36\%).
\maarten{Add a pointer to the appendix with more of these analyses?}
% \jimin{todo: correlation / results by demographics? ask in meeting what's important}

\begin{figure*}[htpb]
  \centering
  \subcaptionbox{Hate speech and counterspeech experiences\label{hate-counter-freq}}{%
     \includegraphics[width=0.45\textwidth]{figures/frequency_hate.pdf}%
  }
  \subcaptionbox{Most Commonly Seen Hate Speech Categories\label{subfig:hate-type}}{%
    \includegraphics[width=0.45\textwidth]{figures/hate_type.pdf}
  }
  \caption{Hate Speech and Counterspeech Experience Responses}
  \label{a-two-column-figure}
\end{figure*}

\subsection{Survey Design}
\maarten{this is a little long, can we potentially give high-level picture and list the questions in a table format or enumarated format?}
The survey was designed after initial qualitative interviews reflecting some of the high-level findings such as AI tools discussed by the experienced counterspeakers. 
% We iteratively designed the survey as a research team.
The survey included four main parts: hate speech experience, counterspeech experience, AI tools for counterspeech, and demographics.
In the first part, we asked the participants questions about social media usage and their experiences with hate speech online such as types of hate, platform, and types of online spaces, public or private (5 questions).
The second part of the survey consisted of questions about counterspeech experience. 
More specifically, we asked participants about their responses to hate speech and barriers to responding if they had chosen not to respond (\todo). 
The third part of the survey focused on questions about AI tools. 

\maarten{The next part is quite long, and feels somewhat redundant}
To understand how open participants were to AI tools more generally, we asked how likely they would be to use an AI tool that assisted solving the barriers they selected. 
We asked two qualitative questions prior to the quantitative questions about tool preferences to prevent any priming of the users with certain types of tools. 
First, we asked participants what the reasons would be to either use or not use an AI tool that addressed their concerns when responding to hate speech. 
Second, we asked participants to envision possible AI tools, if any, that might make them more likely to write a response to hate speech. 
Below is the specific wording for each qualitative question.
\begin{enumerate}
    \item What are the reasons that you are likely or unlikely to use it (an AI tool that addresses the barrier in the previous questions)?
    \item What type of AI assistance do you think would make you more likely to write a reply to hate speech?
\end{enumerate}
In the quantitative portion, we divided tools envisioned by the research team and the experienced counterspeakers into two types: collaborative writing tools for counterspeech and bots, i.e., automated responses. 
\jimin{probably need to remove that some options were from the interview since we don't specify how}
% add something here about the questions that were either choose all that apply or choose three

\subsection{Analysis Method}

\paragraph{Quantitative Responses}
We report the quantitative responses with percentage of participant responses. 
For those questions that asked participants to select all that apply, we counted the number of participants who responded and calculated the percentage.

\jenny{Maybe be more specific about how you calculate the percentage? Are we aggregating similar responses together (e.g., strongly agree, agree)? For each type of Likert response, we could describe which categories we combined together / what we end up reporting in our results in the \%s.}\maarten{+1}

\paragraph{Qualitative Responses}
\maarten{This is quite long, can we break this up into paragraphs, and maybe condense?}\jenny{tried giving it a go on condensing/splitting into paras, thoughts?}

To analyze the qualitative survey responses, we performed open coding on the data. In this analysis, we interpreted generated codes as itemized claims about the data to be investigated in other work and surfaced coding disagreements, following recent best practices in qualitative analysis~\cite{hammer2014confusing}. 

To open code the data, separate documents containing the survey responses to each question were created~\cite{saldana2009coding}. Next, two authors first inductively generated codes for 25\% of the data by developing individual code books and labeling each instance with zero ore more codes. Each code was given a name along with a short description. Next, the authors convened to merge their individual codebooks into a shared codebook. The authors first identified codes with similar themes and merged them into a single code. For the remaining codes, the authors discussed instances of disagreement and unanimously agreed to add, merge, or delete the code from the codebook. 

Finally, the authors performed a second round of coding by deductively applying the shared codebook to the entire dataset individually. The authors then reconvened to apply the codes. For each instance in the dataset, the authors applied the codes they both agreed upon and discussed the disagreements on others. They added or removed the code from the instance upon unanimous agreement. Disagreements largely occurred due to differing scopes of codes and at times different interpretations of the statements, which were resolved through discussion.

% \subsection{Quantitative Results}
% \jenny{Can we move this section to findings instead?}

% \paragraph{Online Hate Speech Experiences}
% When asked about their online hate speech experiences, overwhelming majority (94\%) of the respondents said they had encountered hate speech online. 
% Facebook and Twitter / X were the top two platforms where participants encountered hate speech most frequently although YouTube and Facebook ranked the top weekly used platforms. 
% Most participants observed more hate speech in public online spaces (84\%) compared to private.

% The types of hate the participants reported seeing most frequently were ``Race-based or Ethnicity-based hate speech'' (56\%) followed by ``Hateful speech against members of a specific political party'' (48\%).
% The full rankings of categories of hate are shown in Figure~\ref{subfig:hate-type}. Additional categories of hate encountered and identified by the participants are listed below. Examples of online hate encountered by participants include \jenny{fill this in with participant quotes}
% \begin{itemize}
%     \item ``against farmers, vegans''
%     \item ``Against people with different entertainment preferences''
%     \item ``General hatred towards liking certain things, like matters of personal taste''
%     \item ``Anti Conservative hate, anti Straight hate, anti male hate''.
% \end{itemize}

% \paragraph{Counterspeech Experiences and Barriers}
% As shown in Figure~\ref{hate-counter-freq}, participants responded to hate speech in much lower rate than encountering hate speech.
% When participants did respond to hate speech, highest number of participants were primarily responding to ``people that they (I) do not know'' (49\%) and ``equally as an ally and as a member of the targeted group'' (45\%).

% % who are they responding to?
% The participants responded to hate speech by almost equally commenting or replying directly under the post (72\%) and reacting with downvotes or dislikes (70\%) followed by reporting hateful speech (49\%). 
% The participants reported that they have responded by using tactics to ``correct misinformation'' (72\%), ``shame the person who posted hate speech'' (36\%), and ``posted links to trustworthy sources'' (34\%). 
% The tactics that participants reported using most often were 
% Some other tactics identified by the participants included the following.
% \begin{itemize}
%     \item ``I think I tend not to post or get involved in a hate speech post.''
%     \item ``I like copying their post, but changing the demographic so they can see how bigoted they are.  Such as all the anti-white racism that I see, I will write an exact copy of their post and put "black" where they had the word "white" and suddenly they think it's "racist". It exposes their own biases.''
%     \item ``be hateful back''  
% \end{itemize}

==> content/backups/06-discussion.tex <==
\section{Discussion}
\jimin{think about why we found this}
\jimin{talk about how to deal with this}
\jimin{structure - one or two sentences relating to what we found, similar work found related things, new paragrph on recommendations maybe AI can help with ...}
% \maarten{I would start this section with a paragraph that summarizes what we did (think conclusion-y), as well as the main findings, and then say we discuss some implications of our findings below.}
% \jimin{addressed}\maarten{Nice job!}
% \maarten{The role of discussion sections is to tie together our findings with other work (that has found similar or related things, or argued for things that we argue for here, etc.)}
% Maarten suggestions: do more bottom up
To answer how AI assistance should be developed to help counterspeaking and not to detract from its meaning, we conducted interviews and surveys with both experienced and inexperienced counterspeakers to investigate three research questions: what are barriers to counterspeaking (RQ1), how could AI tools assist in counterspeech (RQ2), and what are some concerns about AI involvement in counterspeech (RQ3).

Our analyses surfaced four different themes or barriers and AI needs to inform functional needs of AI assistance and found that many participants thought AI tool could be empowering. 
Moreover, we discovered themes of counterspeaker motivations, especially in connection to self and others, highlighting the human components of counterspeech. 
Through understanding participants' concerns of AI involvement, we identified that without careful considerations, AI tools could do more harm than good, detracting from counterspeaker motivations and reducing meaning in communication.  
Based on our findings we build a set of recommendations and considerations for designing beneficent AI tools for counterspeech.

\maarten{Idea on re-structuring:
as it is, the distinction between the subsections isn't super clear; many design considerations are related to the authenticity and meaning piece, and we probably don't need more than a paragraph for the policy recs ... I would just merge/remove all the subsections, and make each point a \textbackslash paragraph; and for discussion items where we have design recs you could maybe have a two-paragraph \textbackslash paragraph (sorry not sure how else to say this haha). Proposed discussion items based on what you have rn: 
- authenticity of communication \& trust
- meaning \& moral imperative
- fatigue and mental health
- policy recs}

\maarten{I like this discussion item, but we need to drive this home a little bit better. We need to make it crystal clear AI counterspeech could get in the way of (1) authenticity of communication and (2) the meaning that people derive from counterspeaking, which is linked to the moral imperative many people feel about counterspeaking being the "right thing to do". TBH i think we should break these two items up into separate subsections / paragraphs. I would also add a LOT more citations about technosolutionism and how AI can remove the authenticity / humanity of certain tasks, and how that's something to be avoided.}
% Maarten: minor, but in general, try to start these paragraphs with high level themes/findings from our paper ( counterspeech is often a moral imperative...)
\paragraph{Authenticity of Communication}

% authenticity makes counterspeech meaningful
% authenticity, therefore, is key to what makes counterspeech effective or meaningful?
% connect concerns of authenticity to previous works - why is it important that counterspeech is authentic? (especially online)
One of the overarching concerns of AI tool participants discussed was authenticity of communication.
Authenticity is a complex social concept rooted in self-understanding and acceptance as well as in openness, sincerity, and truthfulness in relational context \cite{kernis2006authenticity}, linked to psychological well-being and relationship quality \cite{Wilt2019-ow,Bailey2020}.
It is also at the core of creating solidarity in activist movements \cite{horowitz2017we}, to organize and participate \cite{SCHULTE2020identity}.
It is therefore, core to counterspeech when those speak up for values they \textit{``stand up for''} (SP223) that it is coming from the true self. 
Thus, the presence of AI tools could in short-term negatively affect credibility of counterspeakers as discussed in \S~\ref{subsubsec:auth-n-agency} and might lead to silencing of counterspeakers' voices due to audience's distrust. 
% trust and activism
% collective identity
In long-term, careless deployment of AI in counterspeech could lead to disengagement due to growing mistrust. 
Moreover, as discovered through participant responses, it takes personal risks to counterspeak opening them up for potential conflict and harm to mental health. 
These risks as well as the emotional, social, and physical distance of online interaction make trust an essential component to both speaker and audience \cite{Hansson2021metoo}.
% cynicism and mistrust lead to civic disengagement - horizontal trust
% talk about meaningful effort here

\paragraph{Design Consideration: Ensuring Trust} 
% AI mediated communication has been shown to reduce trust and authenticity is really important for counterspeech
Building trust is a key consideration for designing AI tools for counterspeech as AI mediated communication has already been shown to negatively affect trustworthiness of the speaker and authenticity of the message \cite{jackesch2019aimc,gilkson2023aimcaplogy}. 
Any system that generates automated counterspeech responses (bots) should clearly disclose that it is not a human \cite{etzioniOpinionHowRegulate2017}. 
Such transparency will help users determine who they are communicating with and will lead to less information overload due to unclear sources \cite{laato2020unverified}.
Another avenue that can help encourage transparency would be bot detection.
However, for responses generated through human-AI collaboration, it is less clear how much disclosure is necessary.
Similar to other AI mediated communication tools which can lead to different perception of the writers and their intentions and feelings of deception \cite{hancock2020aimc,Hohenstein2023-zj}, AI counterspeech and its closeness to morality and personality may lead to further. 
Therefore, it is an important research direction to understand how to communicate and present communication that is collaboratively created with AI.

% might add into the section
% The politeness and positivity bias in AI mediated communication can exacerbate the already positive biased social media interaction and discourage people from showing complex emotions.
% \textit{``keyboard warrior''} (SP333)
\jimin{also something about being transparent with failure / bot detection}

\maarten{I'm not sure what you're trying to say in this paragraph here? there's a lot of independent points that you make, but what is the main claim, and how are the other claims connected to that main claim? part of this is about improving the discourse flow as well} \jimin{tried to address} \maarten{Also a good place to echo the "protesting robots" title?} 
\paragraph{Moral Imperative}
% morality shifting and protesting robots
Many participants saw counterspeech as a moral imperative believing that it was the \textit{``right thing to do''} (IP1) and a \textit{``simple duty I could fulfill''} (SP266).
Participants chose to counterspeak against hate on topics that they cared about or valued. 
For example, one participant said that counterspeaking on \textit{`topics that we are passionate about keeps me going''} (IP3).
Counterspeech, thus, was an important tool to express one's morality and a tool to guide correct perception of group moral attitudes \cite{friessCollectiveCivicModeration2021,hanCivilityContagiousExamining2018} which is key to a functioning democracy \cite{Rini2019-RINSMD,Brady2023}.
However, social media platforms and technologies have the power to amplify incorrect portrayals of moral attitudes \cite{Brady2023,brady2021outrage}, in line with a reflection shared by IP5: 
\begin{quote}
    \textit{``You already have this impression that everyone is right wing extremism, but no, that’s not true, it’s a very small minority.''}
\end{quote}
Therefore, conveyance of morality, norms, and values should be considered carefully within counterspeech research and the impact of AI systems to internal and external understanding of morality, especially in the context of their biases and failures, requires further investigation.
\maarten{I don't fully understand the role of this subsection on morality.. I know that this was a theme that we found a lot, but some of the discussion items feel a little far fetched? I think we can just merge the main point (ie. that counterspeech is often a moral imperative) into the design consideration below, and delete this subsection?}
% Delegation of unethical activities to AI has been proposed as a direction of research \cite{kobis2021morals}.
% However, delegation or partnership in ethical behaviors would also be an important future direction to address AI involvement in moral actions: how can AI tools augment without detracting meaning and without taking away or overly exerting humanness. 
% collective and personal identity

% something about ai mediated communication here?

% what are the different perspectives to offer here that is not in the findings? 
% We kind of concluded that there are goods and bads of ai in counterspeech here we can expand further on ??

% I think a good conclusion and next direction would be to identify meaningful / non-meaningful effort - finding fact seems not as meaningful to people (?)

% questions around what does it mean to outsource moral action and civic engagement? Does that make us less human? 
% dehumanization

% risk-shifting / morality-shifting

% \paragraph{Internal and external}

% \paragraph{Short term and long term}
% \subsection{Educational}


% maybe move to the structural need section
% \subsection{Different Definitions of Effective Counterspeech}
% emotions?
% unbiased?
% maybe the biggest difference here
% general public 
% - audience is usually the person who posted (try to change their mind)
% - thinks factual / logical responses are best
% - are more ok with bots 
% - most rewarding: even just one person
% 
% The level of engagement of AI tool that was preferred by users varied the most between experienced counterspeakers and wider public.
% \subsection{Design Considerations}
% Despite the concerns listed above, many of our participants still thought that AI tools would be empowering, especially in confidently standing up against hate against increasing amount of polarization and hate as well as fear speech in social media. 
% Here we discuss considerations that are key to design of counterspeech AI tools. 
% \jimin{also mention designing around algorithms if for social media?}
% one of the most useful tool can be a bot detection tool?

\paragraph{Design Consideration: Preserving Moral Agency}
% \jimin{will add more citations}
% ai assistance in counterspeech can take away moral agency and even worse suggest unethical replies
% these unethical replies can be delegated to AI to post
% how to preserve moral agency? - need to focus on context situated for deployment, make personalizable / customizable answers, take responsibility? 
\maarten{I'm not sure I fully understand what this subsection is trying to say? again, the main point to me is that (1) counterspeaking is often a moral imperative for people who do it, so (2) AI systems should take that into account and be designed such that the agency---moral or otherwise--- and value diversity of counterspeakers are preserved, cause otherwise counterspeakers might stop doing it (make an analogy to other tasks that AI could "ruin" for people) and/or the diversity of moral values expressed in counterspeech could be lost (cite some work on cultural biases in AI systems)?}
As noted above, counterspeech is closely related to morality of the counterspeaker.
Therefore, preserving moral agency is a key design consideration as AI tools have been shown to alter moral decisions \cite{Krugel2023-sg}.
There, however, are different levels of moral disagreements in countering different types of hate speech, notably misinformation.
Based on the common ground that the value of truth is greater than lies \cite{MacKenzie2020} in many or all context, counterspeech tool to counter misinformation could lead to less moral disagreement.
Thus, understanding the moral reasoning behind countering types of hate would help resolve moral disagreements and distinguish meaningful effort from those less meaningful \cite{INZLICHT2022effort} in the design of counterspeech AI tool. 
Moreover, to address the individual agency of counterspeaking, it would be essential to acknowledge the differences not only in morality but also in definitions of effectiveness.
There is no one solution to this problem, but focusing on creating unbiased systems that can be more easily aligned with users through personalization or customization of output would be recommended. 
% As one participant said, 
% \begin{quote}
%     \textit{``I would like to have the support of the tool, and to be honest it sort of makes me feel like I have some plausible deniability if an issue arises. In a worst case scenario I would be able to "blame" it on the AI.''} (SP277)
% \end{quote}
% \textit{``Other than assistance with grammar and spelling I don't think I would use an AI for something as important as taking a stand against hate.''}
\jimin{deployed within cultural and global context}
AI generated text can instill values and norms \cite{Krugel2023-sg,Jakesch_2023} that may encode biases \cite{weidinger2021llmharm,farina2023gptissue} or only reflect values of specific cultures \cite{santy-etal-2023-nlpositionality} leading to further marginalization and can reduce the opportunity for people to bring authentic emotions into conversations \cite{Hohenstein2023-zj}.
% recommendations for fact-checking tool?

\paragraph{Mental Health}
The \textit{``stress''} (SP112) of responding and \textit{``not caring enough''} (SP30) were frequently shared by participants. 
Experienced counterspeakers also noted that constant exposure to hate speech and call for action can lead to feelings of being \textit{``overwhlemed''} (IP3) and \textit{``becoming too much''} (IP5).
This is consistent with literature on experience of cyberbullying victimization, becoming the target of cyber harassment or hate speech, and its link to mental health, especially in depression, anxiety, and social media fatigue \cite{schodt2021cyber,cao2019smf,JENARO2018cyber}.
Mental health of those who are being countered should also be taken into consideration as counterspeech can also involve online shaming behaviors \cite{Thomason2021shame} and domination \cite{whitten2023republican}. 
\maarten{I'm unsure what the main takeaway is here? Counterspeech can take a toll on those who do it? can we link it to the design consideration below, in saying that if counterspeech takes a mental toll, then more counterspeech cause AI assistance means more risks of a mental toll?}

\paragraph{Design Consideration: Promoting Healthy Engagement}
Tools that are finding hate speech or offering responses should avoid adding unnecessary information for the users and audience who are already overwhelmed \cite{ZHENG2021fatigue}.
One helpful direction would be to help users be mindful and regulate their emotions when responding or after seeing hateful speech. 
Moreover, many counterspeakers engaged to help the victims of hate speech, and previous work has shown that the identity of the sender had an impact on its helpfulness \cite{HighAndrewC2018Scfb}. 
Therefore, the identity and perception of AI as a sender and its impact should also be explored.

\jimin{look up stuff about mental health and ai}
% 

% disclosure and transparency when using a bot - never try to pretend to be a human but how much disclosure? future study
% fact-based and leave room for human connections / emotions?
% unbiased building trust
% educational tool - help people walk through to design a campaign
\paragraph{Policy Recommendations}
\maarten{My current guess is that we might not want a separate subsection for this, but instead maybe have a paragraph? or maybe we want to just remove this section?}
\jimin{tbd}
\begin{itemize}
    \item Disclosure policy around bots \& machine generated texts
    \item misinformation
    \item retaliation
\end{itemize}
% Disclosure policy 
% misinformation
% retaliation

% three rule of AI - robot should never pretend to be a human 
% Access now
% human rights perspective of AI
% ask Nicole for some pointers

% meaningful vs non-meaningful effort of people
% intersting two sides of the story: practical + authenticity and meaning
% design + ethical considerations - I feel uncomfortable with this; the troll farms use this technology introspective side (whether the technology exists, for counterspeaker who do this all the time, it is a moral activity - important civic duty)
% - morality was what they wanted to talk about

% factual things are clearly wrong - so people are more likely to respond, but when it comes to matter of opinion, and the level of what people consider opinions vary, so people are not as sure about this - why we need varied tools since this is a moral decision and what people believe in might be different?

% assessing impact might also become a type of information overload
